Method Calls Frequency-Based Tie-Breaking Strategy For Software Fault Localization

In Spectrum-Based Fault Localization (SBFL), a suspiciousness score is assigned to each code element based on test coverage and test outcomes. The scores are then used to rank the code elements relative to each other in order to aid the programmer during the debugging process when seeking the source of a fault. However, probably none of the known SBFL formulae are guaranteed to produce different scores for all the program elements, hence ties emerge between the code elements. Based on our experiments, ties in SBFL are prevalent: in Defects4J, 54-56% of buggy methods are members of ties, i.e., there is at least one other method with the same score in these cases (but typically much more, on average 6), and this inevitably reduces the effectiveness of any SBFL approach. In this work, we present a technique to break ties in such cases based on the so-called method calls frequencies. This counts the number of different contexts of method calls (both as callees and as callers) in failing test cases. The intuition is that if a method appears in many different calling contexts during a failing test case, it will be more suspicious and get a higher rank position compared to other methods with the same scores. This method can be applied to any underlying SBFL formula, and can favourably break the occurring ranks in the ties in many cases. The experimental results show that our novel tie-breaking strategy achieved a significant reduction in both size and number of critical ties in our benchmark. In 72-73% of the cases, the ties were completely eliminated and the average reduction rate was more than 80%.

==> table_average_diffs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[H]
	\caption{Improvements of average rank}
	\label{tab:avg_improvements}
	\centering
	\resizebox{1.0\columnwidth}{!}{
	\begin{tabular}{c|cc|cc|cc|cc|cc}
	\multirow{2}{*}{} & \multicolumn{2}{c|}{\sconf} & \multicolumn{2}{c|}{\sdstar} & \multicolumn{2}{c|}{\gpA} & \multicolumn{2}{c|}{\sochiai} & \multicolumn{2}{c}{\starantula} \\
	& diff        & \%         & diff        & \%          & diff       & \%        & diff       & \%         & diff       & \%         \\
	\toprule
	Chart             & -0.58       & -1.69      & -0.58       & -6.32       & -0.58      & -1.69     & -0.62      & -7.03      & -0.44      & -2.76      \\
	Lang              & -0.34       & -7.47      & -0.37       & -8.30       & -0.34      & -7.74     & -0.35      & -7.85      & -0.32      & -6.18      \\
	Math              & -0.29       & -2.68      & -0.41       & -4.00       & -0.29      & -2.68     & -0.43      & -4.17      & -0.41      & -4.02      \\
	Mockito           & -0.15       & -0.49      & -0.15       & -0.58       & -0.14      & -0.33     & -0.15      & -0.58      & -0.15      & -0.57      \\
	Time              & -0.19       & -0.90      & -0.19       & -1.02       & -0.19      & -0.83     & -0.23      & -1.25      & -0.21      & -1.06      \\
	Closure           & -2.29       & -3.05      & -2.32       & -3.24       & -2.37      & -2.48     & -2.33      & -3.25      & -2.28      & -2.87      \\
	\bottomrule
	all               & -1.11       & -2.84      & -1.17       & -3.25       & -1.15      & -2.36     & -1.17      & -3.28      & -1.14      & -2.87     
	\end{tabular}}
\end{table}

==> table_avg_diffs.tex <==


% we use only 'diff' cases in avf diff calc.
\begin{table}[H]
	\caption{Differences between \enquote{classic} ranks and \enquote{tie-break} average ranks}
	\label{tab:diffs}
	\centering
	\resizebox{0.9\columnwidth}{!}{
	\begin{tabular}{c|cc|cc|cc}
		\multirow{2}{*}{} & \multicolumn{2}{c|}{min} & \multicolumn{2}{c|}{avg}          &\multicolumn{2}{c}{max}          \\
		& diff      & avg diff    & diff   & avg diff & diff    & avg diff \\
		\toprule
		\sconf       & 300.5 & 2.18 & -458.0 & -2.65 & -1216.5 & -5.99 \\
		\sdstar      & 315.5 & 2.17 & -479.5 & -2.70 & -1274.5 & -6.10 \\
		\gpA         & 328.0 & 2.38 & -471.5 & -2.73 & -1271.0 & -6.26 \\
		\sochiai     & 302.5 & 2.18 & -481.5 & -2.75 & -1265.5 & -6.20 \\
		\starantula  & 364.0 & 2.55 & -467.0 & -2.61 & -1298.0 & -6.32 \\
	\end{tabular}
	}
\end{table}




==> table_ranks_in_ties.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[H]
	\caption{Average rank positions in critical ties}
	\label{tab:rank_diff_in_nonOptimal_bugs}
	\centering
	\resizebox{0.9\columnwidth}{!}{%
	\begin{tabular}{r|ccc|ccc}
		\multirow{2}{*}{} & \multicolumn{3}{c|}{\textit{\enquote{before-ties}}} & \multicolumn{3}{c}{\textit{\enquote{after-ties}}} \\
	 	             & \begin{tabular}[c]{@{}c@{}}without\\tie-break\end{tabular}      & \begin{tabular}[c]{@{}c@{}}with \\tie-break\end{tabular}     & diff     & \begin{tabular}[c]{@{}c@{}}without\\tie-break\end{tabular}     & \begin{tabular}[c]{@{}c@{}}with\\tie-break\end{tabular}     & diff     \\
        \toprule
		\sconf       & 55.2        & 53.1      & -2.1     & 45.8       & 43.5      & -2.3     \\
		\sdstar      & 46.9        & 44.8      & -2.1     & 39.3       & 37.0      & -2.3     \\
		\gpA         & 68.8        & 66.7      & -2.1     & 54.0       & 51.7      & -2.3     \\
		\sochiai     & 46.9        & 44.8      & -2.1     & 40.3       & 37.9      & -2.4     \\
		\starantula  & 50.4        & 48.3      & -2.1     & 46.5       & 44.1      & -2.4    
	\end{tabular}
	}
\end{table}

==> tie_observation.tex <==
\section{Observations}
\label{observations}


\todoi{observations}
\todoi{I have no idea - maybe: relation between the fl algs. based on ties (and results)}
\todoi{it depends on the fl-results}
\todoi{@Arpad Answer to RQ4, I don't think this depends on results}


==> tie_survey.tex <==
\section{Ties in Fault Localization}
\label{ties_problem}

\todoi{mini-survey about ties}
\todoi{definitions: tie, critical tie}
%\todoi{new def: the best critical tie}

When program components are ranked using fault localization formulae, it is possible that more than one component gets the same suspiciousness score. For example, all the statements inside a conditional branch could get the same suspiciousness score. Thus, such statements get tied in the ranking and cannot be differentiated from each other in terms of which one has to be examined first. Therefore, tie-breaking strategies are required to break these ties. Tie-breaking strategies are not only important to measure the effectiveness of a fault localization formula, they are also important for comparing formulae with each other. For example, comparing two formulae that each produces a different tie number, type, and size would not give accurate results.

Tied statements are usually broken and ranked based on three approaches ~\cite{ref3} as follows:
\begin{itemize}
\item	MIN measure (also known as the worst case): It refers to the bottom most position of the statement that shares the same suspiciousness value as the other statement(s).
\item	MAX measure (also known as the best case): It refers to the top most position of the statement that shares the same suspiciousness value as the other statement(s).
\item	MID measure (also known as the average case): It refers to the average of the position of the statements that share the same suspiciousness value and it is calculated using Equation 1.
%\[MID=S + (\frac{E-S}{2})\]

\begin{equation}
	\begin{split}
		\text{MID Measure} & = S + \left (  \frac{E - S}{2}\right )
	\end{split}
\end{equation}

Where S is the tie starting position and E is the tie end position. It is worth noting that the MID measure considers the average of all possible positions, therefore; it is more widely used than the other two tie-breaking approaches.\\
\end{itemize}
However, these approaches do not take into account other suspiciousness factors derived from the context in the ranking. It is quite frequent that ties include faulty statements and it is not limited to any particular localization technique or target program. As a result, such statements are tied for the same position in the ranking. Also, it gives an indication that the used technique cannot distinguish between the tied statements in terms of their likelihood of being faulty. Thus, no guidance is provided to developers on what to examine first ~\cite{ref4}. In addition, the greater the number of ties involving faulty statements, the more difficult it is to predict at what point the faulty statement will be found during the examination. Ties can be divided into two types: non-critical and critical. Non-critical ties refer to the case where only non-faulty statements are tied together for the same position in the ranking. Here, if the tied statements have a higher suspiciousness than the actual faulty statement, then every statement will be examined before finding the faulty statement which is considered as a problem. On the other hand, if the tied statements have a lower suspiciousness than the actual faulty statement, then the faulty statement will be examined before the tied statements. Thus, there is no need to continue examining the ranking. In the last case, the internal order in which the tied statements are examined does not affect the performance of fault localization in terms of the number of statements that must be examined before finding the faulty statement. Whereas, critical ties refers to the case where a faulty statement is tied with other non-faulty statements ~\cite{ref4}. In this type, the internal order of examination affects the performance. It is worth mentioning that critical ties are not a rare case in fault localization. Besides, a significant portion of the statements in the program under consideration might be critically tied.
